Quantum Computing: An Overview Across the System Stack

Quantum computers, if fully realized, promise to be a revolutionary technology. As a result, quantum computing has become one of the hottest areas of research in the last few years. Much effort is being applied at all levels of the system stack, from the creation of quantum algorithms to the development of hardware devices. The quantum age appears to be arriving sooner rather than later as commercially useful small-to-medium sized machines have already been built. However, full-scale quantum computers, and the full-scale algorithms they would perform, remain out of reach for now. It is currently uncertain how the first such computer will be built. Many different technologies are competing to be the first scalable quantum computer.

==> content/recent.tex <==
%\section{Recent Advancements and Trends}
%\begin{itemize}
%    \item Typically advancements in last 12 months
%    \item NISQ designs and applications
%    \item Emphasis on changes that happened sooner than %expected (Google's 72- and IBM's 50- qubit computers
%    \item Rhode Island Startup
%\end{itemize}



%\subsection{Fully-Functional Computers}


%\subsection{Hardware Architecture and Devices}
%As the field is nearing practical physical implementations, there is much anticipation on the architecture and device side. If a more reliable quantum device or a scalable architecture is found, it may be the tipping point. The authors of \cite{fu2018microarchitecture} (building on their previous work \cite{fu2017experimental}) present what they believe to be a scalable architecture. They note that most quantum research focuses at the highest (software) and lowest (hardware) levels, which often does not consider the constraints imposed by the other. Their architecture attempts to find a way to combine the two in a scalable manner. A key contribution of this work is separating the non-deterministic (and possibly out-of-order) classical control processor from the quantum operations, which must be in order and at precise times. A related work \cite{fu2018eqasm} developed an instruction set architecture (ISA) targeting the same platform. This ISA could break quantum instructions into more primitive micro-operations, which could be precisely scheduled by the architecture in \cite{fu2018microarchitecture}. \cite{pechal2018superconducting} proposed a superconducting architecture that uses nanomechanical resonators for storage. The resonators are based on phononic crystal cavities, which are compact and have a long lifetime. Multiple resonators that can connect to each qubit. To perform computation on a quantum state stored in a resonator, a swap gate is performed between the resonator and its adjacent qubit. Once in the qubit, it can interact with other qubits in the system. This likens the qubit to a processor and the resonators to on-chip memory. 
%Topological quantum computing is a unique approach as it protected from noise due to the non-locality of the quantum information. A two-qubit programmable quantum computer using quantum dots was demonstrated in \cite{watson2018programmable}.


%Qubits exist as anyons which are held in 1-D Nanowires and computation is performed by braiding their worldlines (moving them around each other in 2-D space) \cite{nayak2008non,alicea2011non} or by performing measurements in a specific order \cite{bonderson2008measurement}. The authors of \cite{friedl2018template} demonstrated large scale growth of InAs nanowires for this express purpose, demonstrating a step towards scalable fabrication for topological quantum computers.

%\subsection{Software}


%\subsection{Algorithms}




%\subsection{Network}


